Neuro-Symbolic Spatio-Temporal Reasoning

Knowledge about space and time is necessary to solve problems in the physical world: An AI agent situated in the physical world and interacting with objects often needs to reason about positions of and relations between objects; and as soon as the agent plans its actions to solve a task, it needs to consider the temporal aspect (e.g., what actions to perform over time). Spatio-temporal knowledge, however, is required beyond interacting with the physical world, and is also often transferred to the abstract world of concepts through analogies and metaphors (e.g., "a threat that is hanging over our heads"). As spatial and temporal reasoning is ubiquitous, different attempts have been made to integrate this into AI systems. In the area of knowledge representation, spatial and temporal reasoning has been largely limited to modeling objects and relations and developing reasoning methods to verify statements about objects and relations. On the other hand, neural network researchers have tried to teach models to learn spatial relations from data with limited reasoning capabilities. Bridging the gap between these two approaches in a mutually beneficial way could allow us to tackle many complex real-world problems, such as natural language processing, visual question answering, and semantic image segmentation. In this chapter, we view this integration problem from the perspective of Neuro-Symbolic AI. Specifically, we propose a synergy between logical reasoning and machine learning that will be grounded on spatial and temporal knowledge. Describing some successful applications, remaining challenges, and evaluation datasets pertaining to this direction is the main topic of this contribution.

==> chapter-dummy/toc.tex <==
\chapter*{Table of Contents}

\begin{enumerate}

  \item \textbf{Introduction ($1$--$2$ pages)}: Here we will gently introduce what Neuro-Symbolic AI is and why it is so important to work in this field; we can keep it very abstract and explain how this paradigm tries to imitate human learning and reasoning, by combining perception, a data-driven process, with reasoning, a logical (and mostly slow) process. \jlnote{We can assume that there is an introduction / preface chapter in the book that stresses the importance of neuro-symbolic reasoning. So I think we can safely skip motivating \emph{general} neuro-symb  olic reasoning. Similar to the book chapter proposal, it would be better to start with motivating spatio-temporal reasoning and then motivating why neuro-symbolic approach is useful for spatio-temporal reasoning.} Then, we will also very gently introduce the spatio-temporal formalisms and cite many application works, and already try to motivate why these formalisms should be used in neuro-symbolic AI, e.g., by saying that spatio-temporal knowledge about the physical reality of the world is sort of \emph{hard} knowledge, i.e., knowledge that is true and verifiable. Finally, we will explain the contributions of this chapter, viz., that we aim to present some successful examples of neuro-symbolic learning and spatio-temporal reasoning integration and how we plan to advance this in the future. \jlnote{The introduction has yet no link to the IJCAI paper~\cite{lee_what_2022} (see also my comment in the Table of Contents Item~\ref{item:1} \textbf{Logic vs Spatio-Temporal Logic}).}

  \item \textbf{Background ($2$--$3$ pages)}: Here we will briefly, yet with sufficient detail, introduce the fields of Neuro-Symbolic AI and Spatio-Temporal Reasoning.

        \begin{itemize}

          \item \textbf{Neuro-Symbolic AI or Learning}: Clearly, the book is on neuro-symbolic AI, so people will already know something about it, but we can use a couple of paragraphs to detail what this framework is, and also provide a very high-level classification of it. The classification would look as follows, and perhaps here we could also mention that our focus is on the third axis of research which aims to retain both symbols and neural network components (\emph{loose} integration, although this term has been used in the past in a bit different way). It is important to note that we do not exclude the other axes of research, but we are symbolic people so this is our strong suit.

                \begin{itemize}

                  \item Neural architectures for logical reasoning\footnote{E.g., W. W. Cohen et al.: \textit{TensorLog: A Probabilistic Database Implemented Using Deep-Learning Infrastructure}. In: J. Artif. Intell. Res. 67 (2020)}

                  % In [12], each clause of a Stochastic Logic Program is converted into a factor graph with reasoning becoming differentiable so that it can be implemented by deep networks

                  \item Logical specification of neural networks\footnote{E.g., G. Sourek et al.: \textit{Lifted Relational Neural Networks: Efficient Learning of Latent Relational Structures}. In: J. Artif. Intell. Res. 62 (2018)}

                  % Lifted relational neural networks [67] is a declarative framework where a Datalog program is used as a compact specification of a diverse range of existing advanced neural architectures, with a particular focus on Graph Neural Networks (GNNs) and their generalisations.

                  \item \jl{Meta-reasoning for task generation.} \jlnote{This is a new class of neuro-symbolic reasoning which appears in \protect\cite{lee_what_2022} and the STRL'22 paper where symbolic intervention is used to prepare the whole dataset. See also Section~\ref{sec:symb-meta-learn} on page~\pageref{sec:symb-meta-learn}.} \msnote{Merge this with the last category and rename the category.}

                  \item \emph{Architectures integrating learning and reasoning}\footnote{E.g., R. Manhaeve et al.: \textit{Neural probabilistic logic programming in DeepProbLog}. In: Artif. Intell. 298 (2021)}
                        \begin{itemize}
                          \item \textbf{\emph{Our main focus here!}}
                        \end{itemize}

                        % Approaches that apply (differentiable) logical inference to compute the consequences of the predictions made by a set of base neural networks. Examples of this sub-class are DeepProblog [41] and Abductive Learning [13].


                \end{itemize}

          \item \textbf{Spatio-Temporal Reasoning}: Here, there will be the usual introduction to spatio-temporal formalisms, but it should be done in a way that will not make the reader want to kill themselves. So, I think we (I) should refrain from the use of terms such as QCNs, or even worse non-associativity, $\omega$-categoricity, and Bodirsky-like terminology. I think ideally we could present spatio-temporal formalisms as a sub-category of knowledge-graphs with certain intuitive transitivity rules that adhere to physics and cognition (provided in the signature of the formalism). Just showing an example of the RCC8 formalism here should be enough. I mean, in the end, we can still be a bit formal about it and have some sort of definition, but we should keep the balance with the previous neuro-symbolic AI section; we can have more details later.

                \jlnote{I agree. This section should provide only the minimum background of spatio-temporal reasoning. Since we also discuss \emph{temporal} reasoning, IA could be introduced in addition to RCC. Furthermore, \protect\cite{lee_what_2022} is based on relative direction. So relative directional relations could also be introduced (cf.~\protect\cite{freksa_formal_2018}).}

        \end{itemize}

  \item \textbf{Neuro-Symbolic Spatio-Temporal Reasoning and Learning ($8$--$10$ pages, $\sim 2$ pages per sub-section)}: Basically, the main section of this chapter. In my humble opinion, I would propose the following sub-sections:

        \begin{itemize}

          \item \textbf{Logic vs Spatio-Temporal Logic}: So, here we should explain $(i)$~why should we bother with trying to encode spatio-temporal knowledge, and $(ii)$~why not just try to encode as much logic as possible (like in Neuro-Symbolic AI), which by default would also contain spatio-temporal knowledge. For point $(i)$, we can make the same argument about how spatio-temporal knowledge adheres to laws of physics and human cognition and is therefore \emph{hard} and verifiable knowledge that an intelligent system should use anyway; here, we can mention causality and some toy examples relating to that. For point $(ii)$, which is the trickier one, I think that we should argue that much of the logic/knowledge should be learned by an intelligent system through its interaction with its environment, so, basically, only a seed, a core, of initial knowledge is needed for that system to be able to generalize, and spatio-temporal knowledge here presents itself as a very viable option and certainly as an option worthy of exploring; here, we can mention how babies how some primitive knowledge about spatial relations, see \url{https://en.wikipedia.org/wiki/Spatial%E2%80%93temporal_reasoning#Influence_from_cognitive_psychology}.

                \jlnote{There is a potential conflict between the need for a core symbolic spatio-temporal knowledge and the IJCAI/STRL papers~\protect\cite{lee_what_2022}, where spatial relations are learned (based on a symbolic intervention for dataset generation) and not hard-coded. To circumvent this conflict, we can propose two different perspectives for neuro-symbolic spatio-temporal reasoning and learning (i) including core symbolic spatio-temporal knowledge in the model; and (ii) designing an environment that teaches spatio-temporal knowledge}

                \msnote{Spatio-temporal knowledge must be a part of data generation as well.}

                \jlnote{Yes, spatio-temporal knowledge must appear in the design patterns of neuro-symoblic spatio-temporal models, either in the model, the training loop or the data generation component.}

          \item \textbf{State of the Art / Related work}: The Semantic Web journal, along with some related workshop papers by Marjan, and some related papers by Mehul

          \item \textbf{Proposed Integration}: Here, we can present all the different options for future work, viz., $(i)$~translate spatio-temporal formalisms to the Luc de Raedt framework, maybe give a small example of what a spatio-temporal formula in DeepProbLog would look like (e.g., instead of handwritten numbers and a rule for addition, we could have images of a yolk and an egg and the rule of \emph{inside}), $(ii)$~translate spatio-temporal formalisms to the NeurASP framework, again maybe show a small example based on that (it is very similar to DeepProbLog, it just uses ASP for the reasoning), $(iii)$~do it natively with a focus on \emph{abduction} (cite many Chinese papers here), basically, extend the formalisms and all the reasoning machinery themselves with probabilities, the hardest option, but worth exploring, basically my IJCAI survey paper together with an ISKE paper.

                \jlnote{We recently published a paper which proposes a general architecture for handling spatial relations~\protect\cite{lee_spatial_2022}. There, we mentioned graph neural networks as an interface for symbolic knowledge. This is not my favorit paper (we wrote the paper mainly to show our collaboration effort with the Tsinghua university in China), but we can mention this paper as well.}


          \item \textbf{Evaluation tools / datasets}: Here, we need to stress the importance of having tools and datasets not only to evaluate the performance of our proposed integration, but also to compare it with pure ML solutions to see what we do better and what we do worse, how are spatio-temporal rules being learned, in what order, what should be delegated to ML and what should be encoded as background knowledge, all this stuff that is very important but also super hard! Basically, your IJCAI paper.

                \jlnote{Yes, this section makes sense and may require some research from us. There are some other datasets for learning relations (e.g., \protect\cite{goyal_rel3d_2020,hong_ptr_2021}), which are mentioned in the IJCAI paper~\protect\cite{lee_what_2022} that we can refer to.}
        \end{itemize}

  \item \textbf{Conclusion and Future work ($3$--$4$ pages)}: Just a wrap-up, and some nice future directions, especially in terms of what the open questions are and how one should go about tackling them.

\end{enumerate}

